Complexity of the Multilevel Critical Node Problem

In this work, we analyze a sequential game played in a graph called the Multilevel Critical Node problem (MCN). A defender and an attacker are the players of this game. The defender starts by preventively interdicting vertices (vaccination) from being attacked. Then, the attacker infects a subset of non-vaccinated vertices and, finally, the defender reacts with a protection strategy. We provide the first computational complexity results associated with MCN and its subgames. Moreover, by considering unitary, weighted, undirected, and directed graphs, we clarify how the theoretical tractability of those problems vary. Our findings contribute with new NP-complete, $\Sigma_2^p$-complete and $\Sigma_3^p$-complete problems. Furthermore, for the last level of the game, the protection stage, we build polynomial time algorithms for certain graph classes.

==> Paper_Version/Undirected_Graphs_weighted.tex <==
\section{Undirected Graphs: the weighted case}\label{sec:undirected_wei}

\subsection{Vaccination-Attack}\label{subsec:undirected_wei_VA}

We first consider the bilevel subgame composed of the vaccination and the attack (infection) phases, i.e., we consider a zero budget for the protection phase. We will prove the $\Sigma_2^p$-completeness of the decision version of this subgame using the bilevel interdiction Knapsack Problem introduced by \cite{DeNegre2011} and proven to be $\Sigma_2^p$-hard in \cite{Caprara2014}. In this bilevel KP, both the leader and the follower can select items in the same set of objects $O$. The aim of the leader is interdict a subset of items, subject to a specific capacity constraint, in order to minimize the total profit of the follower. The items $o\in O$ have a weight $a_o$ and a profit $p_o$. The capacity of the leader is $A$ and the one of the follower is $B$. We define the binary variables $x_o$ and $y_o$, equal to one if the follower (respectively the leader), selects item $o\in O$. The MILP for this problem can be written:
\begin{subequations}
\begin{alignat}{4}
\text{Minimize} \quad
 & 
 \sum_{o\in O}b_oy_o
 &\\
\text{s.t.}\quad & \sum_{o\in O}a_ox_o\leq A& \\
& \text{max}\ \sum_{o\in O}p_oy_o \qquad \text{s.t.}\quad & \sum_{o\in O}p_oy_o\leq B \\
& & y_o\leq 1-x_o & \qquad \forall\ o\in O.
\end{alignat}
\label{DeNeg}
\end{subequations}
The decision version of this problem can be stated as follows: given a set of items $O$, a set of integer weights $a_i$ and profits $p_o$ for such items $o\in O$, a maximum weight capacity $A$ for the leader and a maximum profit $B$ for the follower, is there a subset $O_l\subseteq O$ of items that the leader can select, with total no more than $A$, such that no subset of items $O_f\subseteq O\setminus O_l$ can be selected by the follower with a total profit more than $\Pi\leq B$.

The decision version of the Vaccination-Attack subgame is the following: given a graph $G=(V,E)$, profits $\alpha_v$, vaccination costs $\hat c_v$ and infection costs $h_v$ for $v\in V$, a maximum vaccination budget $\Omega$ and a maximum infection budget $\Phi$, is there a subset of nodes $D\subseteq V$ that the leader can protect, with $\hat c(D)\leq\Omega$, such that for any subset of infected nodes $I\subseteq V\setminus D$ with $h(I)\leq\Phi$, the total weight of the nodes which are not infected is larger than $W$.

\begin{thm}
The decision version of the Vaccination-Attack subgame of the MCV is strongly $\Sigma_2^p$-complete, even if the graph is a tree.
\end{thm}
\begin{proof}
We prove the above theorem by a reduction from the decision version of the DeNegre Knapsack Interdiction Problem (KIP) of model \ref{DeNeg}. We start from a standard instance of the decision version of the DeNegre KIP as defined above. We then construct an instance of the decision version of the Vaccination-Attack subgame as follows. First we construct a star graph $T=(V,E)$ with a central node $r$ and $n$ leaf nodes $v_o$ with $o\in O$ and an edge $\{r,v_o\}$ for each such leaf node. The central node has profit $b_{r}=\sum_{o\in O}p_o+1$ and weights $\hat c_{r}=h_{r}=1$. Each leaf node $v_o$ with $o\in O$ has $b_{v_o}=h_{v_o}=p_o$ and $\hat c_{v_o}=a_o$. Finally, we fix $\Omega=A+1$, $\Phi=B$ and $W=2\sum_{o\in O}b_i+1-\Pi$. In order to obtain a MinMax problem instead of a MaxMin, we can consider the infected nodes instead of the saved nodes. Indeed, the attacker is trying to minimize the number of saved nodes, which is akin to maximizing the number of infected nodes.

Suppose first that the DeNegre KIP decision instance is a \emph{Yes} instance and the set solution set of items is $O_l\subseteq O$ with total weight $a(O_l)\leq A$. Then in the Vaccination-Attack subgame, the leader can select the subset of nodes $D=\{r\}\cup\{v_o:\ o\in O_l\}$ with a feasible vaccination cost $\hat c(D)=1+a(O_l)\leq A+1=\Omega$. Now, the follower can only attack nodes in $\{v_o:\ o\notin O_l\}$ and each node which is not infected will be saved, since the central node of the star graph is vaccinated. The aim of the follower is therefore to select the subset of nodes of maximum total profit which respects the infection budget $\Phi$. Suppose there is a subset $I\subseteq V\setminus D$ for which $\sum_{v\in V\setminus I}b_{v}=2\sum_{o\in O}p_o+1-\sum_{v\in I}<W$, then we can define a subset $O_f=\{o\in O:\ v_o\in I\}\subseteq O$ such that $\sum_{o\in O_f}p_o=\sum_{v_o\in I}b_{v_o}>\Pi$, which is a contradiction. Therefore, the Vaccination-Attack subgame decision instance is a \emph{Yes} instance.

Now suppose that the Vaccination-Attack subgame instance is a \emph{Yes} instance. It means there exists a subset $D\subseteq V$ of vaccinated nodes such that there is no subset $I\subseteq V\setminus D$ of infected nodes for which we have strictly less than a total profit $W$ of saved nodes. Since $\Pi\leq\sum_{o\in O}p_o$, we need to save the central node $r$ in order to achieve a sufficient total profit. Therefore, the infected nodes will be only the nodes $I$ which are directly infected. If we suppose that the DeNegre KIP decision instance is a $No$ instance, i.e., for any set $O_l\in O$ of objects selected by the leader there exists a set $O_f\subseteq O\setminus O_l$ for which $\sum_{o\in O_f}p_o>\Pi$. This means that for any set $D$ of vaccinated nodes which has $\hat c(D)\leq\Omega$, a subset $I=\{v_o\in V:\ o\in O\setminus O_l\}$ with $O_l=\{o\in O:\ v_o\in D\}$ exists, which has $h(I)=p(O_f)\leq\Phi$ and $b(V\setminus I)=2\sum_{o\in O}p_o+1-\sum_{v\in I}b_v<2\sum_{o\in O}p_o+1-\Pi=W$, which is a contradiction. Therefore, the DeNegre KIP decision instance is a \emph{Yes} instance.

This completes the proof that the decision version of the Vaccination-Attack subgame is $\Sigma_2^p$-complete. Moreover, since the DeNegre KIP was shown to be NP-complete even for unary encoding, we can conclude that no pseudopolynomial-time algorithm exists to solve the Vaccination-Attack subgame. Finally, this a star graph is a tree, the problem is $\Sigma_2^p$-complete even on trees.
\end{proof}

\subsection{Attack-Protection}\label{subsec:undirected_wei_AP}

Using a similar reduction to the one above, we can also prove the $\Sigma_2^p$-completeness of the decision version of the Attack-Protection subgame.

\begin{thm}
The decision version of the Attack-Protection subgame of the MCV is strongly $\Sigma_2^p$-complete, even if the graph is a tree.
\end{thm}
\begin{proof}
An instance of the decision version of the Attack-Protection subgame consists in a graph $G=(V,E)$ where each node $v\in V$ has a saving profit $b_v$, an infection cost $h_v$, protection cost $c_v$, a total infection budget $\Phi$, a total protection budget $\Lambda$ and a maximum threshold of saved nodes weight $W$. Its aim is to find and infection $I\subseteq V$ with $h(I)\leq\Phi$ such that for each protection subset $P\subseteq V\setminus I$, the total profit of saved nodes cannot be more than $W$.

Starting from an instance of the decision version of the DeNegre KIP, we construct an instance of the decision version of the Attack-Protect subgame as follows. We first build a star graph $T=(V,E)$ with a root node $r$ and a node $v_o$ for each $o\in O$ linked to $r$ through an edge $\{r,v_o\}\in E$. We set $b_r=\sum_{o\in O}p_o+1$ and $h_r=c_r=1$. We also set $b_{v_o}=c_{v_o}=p_o$ and $h_{v_o}=a_o$ for each $o\in O$. Finally, we set $\Phi=A$, $\Lambda=B$ and $W=P$. From such a reduction, it is obvious that the attacker in the Attack-Protect problem will attack at least the central node $r$, provided that $\Phi\geq 1$, given that it is always more profitable to attack it (and save it for the defender) than any other subset of nodes. Once the central node is attacked, all other nodes which are subsequently protected will \adel{not} be infected. Therefore, the rest of the attack budget is spent on nodes that the attacker wants to forbid the defender to save. This is exactly the setting of the DeNegre KIP and one can easily complete the proof of equivalence of the two decision instances following a path very similar to the proof of the Section~\ref{subsec:undirected_wei_VA}.

As a consequence, we can conclude that the decision version of the Attack-Protect problem is $\Sigma_2^p$-complete and that no pseudopolynomial algorithm exists to solve it. Since a star graph is a tree, the result stated above holds.
\end{proof}
